Analog Physical-Layer Relay Attacks with Application to Bluetooth and Phase-Based Ranging

Today, we use smartphones as multi-purpose devices that communicate with their environment to implement context-aware services, including asset tracking, indoor localization, contact tracing, or access control. As a de-facto standard, Bluetooth is available in virtually every smartphone to provide short-range wireless communication. Importantly, many Bluetooth-driven applications such as Phone as a Key (PaaK) for vehicles and buildings require proximity of legitimate devices, which must be protected against unauthorized access. In earlier access control systems, attackers were able to violate proximity-verification through relay station attacks. However, the vulnerability of Bluetooth against such attacks was yet unclear as existing relay attack strategies are not applicable or can be defeated through wireless distance measurement. In this paper, we design and implement an analog physical-layer relay attack based on low-cost off-the-shelf radio hardware to simultaneously increase the wireless communication range and manipulate distance measurements. Using our setup, we successfully demonstrate relay attacks against Bluetooth-based access control of a car and a smart lock. Further, we show that our attack can arbitrarily manipulate Multi-Carrier Phase-based Ranging (MCPR) while relaying signals over 90 m.

==> revision_plan.tex <==
We will clarify the effect of interference (in-band and out-band) at the end of Section 3.3 and mention explicitly that we utilize a bandpass filter on the power detector input. Further, we will add a remark that smartphones typically do not simultaneously transmit Bluetooth and Wi-Fi signals. (Reviewer A) (done)

We will comment on the factors determining the maximum relaying distance (depending on relay transmission loss (cable), amplification, and wireless channel losses) in Section 3.3. (Reviewer B) (done)

In the Appendix, we will briefly discuss the use of circulators in view of our current setup. We will further mention circulators in Section 6.2.  (Reviewer B)

We will clarify the need for synchronization when comparing our attack to [40]. Our attack requires a coarse timing alignment to the ranging tones but no alignment on the carrier-phase level (i.e., generation of a coherent RF carrier). (Reviewer B)

We will add a comment on the attack implementation as shown in Fig. 6. The figure shows how we implemented the setup in hardware which was sufficient to realize signal manipulation for MCPR and reciprocity. However, the attenuator and phase shifter could also be inserted in arbitrary other configurations into the signal paths. (Reviewer B)

We will add a comment that we used Eqs. (3) and (4) to obtain the results shown in Fig. 8 (we did not adjust the attacker setting to achieve a specific desired distance). Further, we will add a remark that Eqs. (3) and (4) consider channel effects (assuming LOS channels with ideal linear phase for all links), implicity covered by incorporating the actual physical node distance d. (Reviewer B)

We will add emphasis in the Introduction that we utilize a phase shifter for the MCPR distance manipulation. (Reviewer C)

We will mention in the differentiation from previous work and in Section 3.2 that unidirectional relay attacks can be defeated by means of challege-response protocols, thus requiring bidirectional relaying. (Reviewer C)

We will remove Figure 4. (Reviewer C) (done)

We will move the differentiation from previous work to the Introduction, before the enumeration of contributions. (Reviewer C) (50\% done, add motivation, state-of-the-art, contribution)

We will mention that our setup is not tied to automotive applications, e.g., Tesla, but is rather generically applicable to TDD 2.4 GHz wireless systems (such as Bluetooth or even Wi-Fi). (Reviewer C)

We will add a comment in the Discussion section towards the possibility of simultaneous GPS spoofing and relaying. We will add a reference on GPS spoofing. (Reviewer C)

We will add a remark that the linear frequency change is not a definitve requirement for MCPR. However, randomized MCPR frequency sweeps are likely to increase measurement time due to increased PLL settling times. Further, we will mention possibilities to measure the current tone frequency (frequency counting, phase/frequency detection) in Section 6.3. (Reviewer C)

In Section 5.3, we will add a remark that the experiments were carried out in an ordinary environment where wireless channels behave rather randomly. Further, we will mention that the wireless channel in the attack setting consists of the concatenation of three channels (wireless, relay, wireless) as depicted in the middle of Fig. 10 (left). We will clarify that the adjustment factor Beta is applied to compensate asymmetries within the relay hardware but not the involved wireless channels.
